Rejoinder to the discussion of "Mode-based estimation of the center of symmetry"

Rejoinder to the discussion by Hino (2025) and Pardo-Fern\'andez (2025) of Chac\'on and Fern\'andez Serrano (2025), a special paper (with discussion) published in Annals of the Institute of Statistical Mathematics.

==> configuration.tex <==

\pagestyle{myheadings}

\makeatletter
\@namedef{subjclassname@2020}{%
    \textup{2020} Mathematics Subject Classification}
\makeatother


\makeatletter
\let\blx@rerun@biber\relax
\makeatother


\addbibresource{main.bib}


\renewbibmacro{in:}{}


\AtEveryBibitem{%
    \clearfield{number}%
    \clearfield{issue}%
    \clearfield{pagetotal}%
    \clearname{editor}%
    \ifentrytype{article}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
    \ifentrytype{book}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
    \ifentrytype{inbook}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
    \ifentrytype{incollection}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
    \ifentrytype{inproceedings}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
    \ifentrytype{manual}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
    \ifentrytype{thesis}{%
        \clearfield{url}%
        \clearfield{urldate}%
    }{}
}

\renewcommand*{\bibfont}{\footnotesize}


\DeclareFieldFormat{postnote}{\mkcomprange[{\mkpageprefix[pagination]}]{#1}}

\DeclareFieldFormat{pages}{\mkcomprange{#1}}
\DeclareFieldFormat[article, periodical]{volume}{\mkbibbold{#1}}

\DeclareFieldFormat[article, inbook]{title}{#1}


\DeclareNameAlias{author}{last-first}


\defbibfilter{references}{%
    type=article or
    type=book or
    type=inbook or
    type=incollection or
    type=inproceedings or
    type=manual or
    type=thesis or
    type=misc or
    type=report
}

\defbibfilter{online}{type=online}
\defbibfilter{software}{type=software}


\makeatletter
\let\blx@rerun@biber\relax
\makeatother

